Conflict and Fairness in Resource Allocation

In the standard model of fair allocation of resources to agents, every agent has some utility for every resource, and the goal is to assign resources to agents so that the agents' welfare is maximized. Motivated by job scheduling, interest in this problem dates back to the work of Deuermeyer et al. [SIAM J. on Algebraic Discrete Methods'82]. Recent works consider the compatibility between resources and assign only mutually compatible resources to an agent. We study a fair allocation problem in which we are given a set of agents, a set of resources, a utility function for every agent over a set of resources, and a {\it conflict graph} on the set of resources (where an edge denotes incompatibility). The goal is to assign resources to the agents such that $(i)$ the set of resources allocated to an agent are compatible with each other, and $(ii)$ the minimum satisfaction of an agent is maximized, where the satisfaction of an agent is the sum of the utility of the assigned resources. Chiarelli et al. [Algorithmica'22] explore this problem from the classical complexity perspective to draw the boundary between the cases that are polynomial-time solvable and those that are \NP-hard. In this article, we study the parameterized complexity of the problem (and its variants) by considering several natural and structural parameters.

==> FFT-basics.tex <==
% !TEX root = main.tex

%\newcommand{\util}{\ensuremath{{\rm u}}}

%\il{(DONE) Taken from EMF....clean it for our present discussion. Replace $|\A|=n$ and $|\I| = m$. }
%
%\il{Move Big picture to Intro ?}
%\todo[inline]{maybe just remove it}
%\noindent{\bf Big Picture:} Any subset $S \sse \I$ can be viewed as a subset of $[m]$. Let $\chi(S)$ denote the characteristic vector of $S$. We view $\chi(S)$ as an $m$- digit binary number. A crucial observation guiding our algorithm is that two sets $S_1$ and $S_2$ are disjoint iff the number of $1$s in $\chi(S_1)+ \chi(S_2)$ (binary sum/modulo $2$) is equal to $|S_1|+|S_2|$. 
%
%%\begin{dontshow}
%
%We recursively define polynomials \polyn{i}{s} for each $i\in [n]$ and $s\in \mathbb{Z}_{\geq 0}$ containing all possible monomials that represent feasible bundles for agents $\{1, \ldots, i\}$ whose total utility\todo{it should be size} add up to $s$. Crucially, the bundles are pairwise disjoint subsets of items whose utility for each agent is at least $\eta$. \todo{not correct}
%This type of representation allows us to succinctly capture the property of disjointness between the subsets of \A, as well as guarantees that every agent gets a non-empty bundle. To see this let us consider disjoint subsets $S_{1}, S_{2} \sse \I$ and note that $y^{\chi(S_{1})} \times y^{\chi(S_{2})} = y^{\chi(S_{1}) + \chi(S_{2})}$. Due to the disjointness of the sets, the characteristic vectors do not have 1 in the same position.  Consequently, $\chi(S_{1}) + \chi(S_{2})$ is also an $m$-length binary string that contains exactly $|S_{1}| + |S_{2}|$ number of 1s. %We only construct polynomials that result from multiplying at most $|\A|$ monomials representing the feasible bundles for every agent.
%
%In the final stage of our algorithm, we look for a value of $s\in \mathbb{Z}_{\geq 0}$, such that $\polyn{n}{s}$ is non-zero. That is, there is a monomial that is generated by multiplying $n$ monomials that constitute $n$ bundles of \I.
%The fact that we never go beyond an $m$-length characteristic vector as the degree ensures that the actually degree of the monomial in terms of decimal is at most $2^{m}$. This allows us to use the $\Oh(d \log d)$ algorithm to multiply two polynomials of degree $d$ (in decimal), \citet{moenck1976practical}. Thus, in this manner we can obtain an algorithm that runs in time $\Oh^{\star}(2^m)$.
%
%\il{upto here may move to Intro}

%\begin{dontshow}


%\end{dontshow}



%\Ma{With a slight abuse the notation, we denote $ \Co{H}(i) = h$.}\ma{need this?}
%}

\begin{observation}\label{obs:disjoint-binary-vectors}
Let $S_1$ and $S_2$ be two binary strings of same length. Let $S=S_1+S_2$. If $H(S)=H(S_1)+H(S_2)$, then $S_1$ and $S_2$ are disjoint binary vectors. 
\end{observation}

% The following is due to Cygan et. al~\cite{DBLP:journals/tcs/CyganP10}.

\begin{proposition}\cite{DBLP:journals/tcs/CyganP10}\label{prop:disjoint-set} Let $S=S_{1} \cup S_{2}$, where $S_1$ and $S_2$ are two disjoint subsets of $[m]$. Then, $\chi(S)=\chi(S_1)+\chi(S_2)$ and $H(\chi(S))=H(\chi(S_1))+H(\chi(S_2))=|S_1|+|S_2|$.
\end{proposition}

Observation~\ref{obs:disjoint-binary-vectors} and Proposition~\ref{prop:disjoint-set} together yield the following. 

%Crucially, we obtain the following.
\begin{corollary}\label{cor:HW-disjointness}
Subsets $S_{1}, S_{2} \sse \I$ are disjoint if and only if Hamming weight of the monomial $x^{\chi(S_1)+\chi(S_2)}$ is $|S_{1}|+|S_{2}|$. 
\end{corollary}
%\todo[inline]{in the definition of Hamming weight, exponent is not binary. So, we shall change the definition.}
%This property is used crucially in our algorithm. 


%\Ma{Moreover, $S_{1}\cup S_{2}$ is a disjoint union if $\Co{H}(\chi(S_{1}\cup S_{2})) =|S_{1}|+|S_{2}|$.} 


The {\em Hamming projection} of a polynomial $p(y)$ to $h$, denoted by $H_{h}(p(y))$, is the sum of all the monomials of $p(y)$ which have Hamming weight $h$. We define the {\em representative polynomial} of $p(y)$, denoted by $\Co{R}(p(y))$, as the sum of all the monomials that have non-zero coefficient in $p(y)$ but have coefficient $1$ in $\Co{R}(p(y))$, i.e., it ignores the actual coefficients and only remembers whether the coefficient is non-zero. We say that a polynomial $p(y)$ {\it contains a monomial} $y^i$ if the coefficient of $y^{i}$ is non-zero. The zero polynomial is the one in which the coefficient of each monomial is $0$. 


Now, we are ready to discuss our algorithm. We focus the algorithm on \pcffa and highlight the required changes for other two variants. 






==> clique.tex <==
%!TEX root = main.tex
%\section{Polynomial time algorithm}

%Due to Theorem~\ref{thm:poly-clique}, we know that the problem is polynomial-time solvable when the \conflict graph is a complete graph (there is an edge between every pair of vertices).

%\begin{comment}
Starting point of our results in this section is the polynomial-time algorithm for \cffa when \conflict graph is a complete graph (there is an edge between every pair of vertices). We give proof of Theorem~\ref{thm:poly-clique}. We begin with a simple observation,  which follows due to the fact that the maximum size of an independent set in clique is $1$. 
\begin{obs}\label{bundlesize-clique}
If the \conflict graph is a complete graph, then the bundle size is $1$. 
\end{obs}
%\end{comment}

\begin{comment}
\begin{proof}[Proof of Theorem~\ref{thm:poly-clique}]
Let $\X{J}=(\A, \I, \{\util_{a}\}_{a\in \A}, \Co{H}, \eta)$  be a given instance of \cffa. In light of Observation~\ref{bundlesize-clique}, we construct the following auxiliary bipartite graph $G=(L,R)$ as follows: for every agent $a\in \Co{A}$, we add a vertex $a$ in $L$ and for every \object $x\in \Co{I}$, we add a vertex $x$ in $R$.  If $p_a(x) \geq \eta$, then add an edge $ax$ in $G$. Next, we find a maximum matching $M$ in $G$. If $M$ does not saturate $L$, then return ``no'', otherwise return the following function $\phi \colon \Co{A}\rightarrow 2^{\Co{I}}$, $\phi(a)=M(a)$. 

Next, we prove the correctness of the algorithm. Clearly, if we return the function $\phi$, then it is a solution as we have an edge $ax$ if and only if  $p_a(x) \geq \eta$ and $M$ is a matching in $G$ saturating $L$. Next, we prove that if $\X{J}$ is a yes-instance of \cffa, then the algorithm returns a function. Let $\phi$ be a solution to $\X{J}$. Since $p_a(\phi(a)) \geq \eta$, we have an edge $a\phi(a)$ in $G$. Thus, there exists a matching in $G$ saturating $L$. Hence, the maximum matching $M$ in $G$ saturates $L$ and the algorithm returns a function. 
\end{proof}
\end{comment}


\subsection{When conflict is highly localized: conflict graph is a cluster graph}\label{ss:cluster-proof}
%Due to Theorem~\ref{thm:hardnessForcluster}, the problem is intractable for cluster graph  even when it consists of $3$ cliques. 
%
%\begin{comment}

As discussed in the Introduction, there can be scenarios, where the incompatibilities are highly localized in a way that the set of \items can be decomposed into these small chunks where there is incompatibilities between all \items in the same chunk and none between \items in different chunks. Such a scenario is captured by a cluster graph 


%\il{Need example: A situation where the "conflict" or "incompatibilities" are highly localized such that the set of \items can be decomposed into these small chunks where there is conflict between all \items and no conflict with \items in different chunks. Such a scenario is captured by a cluster graph. (Done)}

We show that the problem is intractable for cluster graph  even when it consists of $3$ cliques. This is in contrast to \Cref{thm:poly-clique}. To show the {\sf NP}-hardness, we give a polynomial time reduction from {\sc Numerical 3-dimensional Matching} problem, which is known to be \nph~\cite{garey1979computers}. In 
\NumMatch\ problem, we are given three disjoint sets $X$, $Y$, and $Z$, each containing $\tilde{m}$ elements, a size $s(a) \in \mathbb{Z}_{+}$ 
for each element $a\in X\cup Y\cup Z$,  and a bound $B\in \mathbb{Z}_{+}$. The goal is to partition $X\cup Y\cup Z$ into $\tilde{m}$ disjoint sets $A_1,\ldots, A_{\tilde{m}}$ such that (i) each $A_{i}$, where $i\in [\tilde{m}]$, contains exactly one element from each of $X$, $Y$, and $Z$, and (ii) for each $i\in [\tilde{m}]$, $\sum_{a\in A_{i}}s(a) = B$. Note that it follows that $\sum_{i\in [\tilde{m}]}\sum_{a\in A_{i}}s(a) = \tilde{m}B$.  Next, we give the  desired reduction.
% in the following theorem. 
%by three multisets of integers $X, Y$ and $Z$, each containing $k$ elements, and a bound $b$. The goal is to select a subset $M$ of $X\times Y\times Z$ such that every integer in $X$, $Y$ and $Z$ occurs exactly once and that for every triple $(x,y,z)$ in the subset $ x+y+z=b$ holds.

%\begin{theorem}
%\cffa is \npc when \Co{H} is a cluster graph containing $3$ cliques.
%\end{theorem}
%\end{comment}


%\begin{comment}

\begin{proof}[Proof of Theorem~\ref{thm:hardnessForcluster}]  Given an instance\\
$\X{J}=(X, Y, Z, \{s_a\}_{a\in X\cup Y \cup Z},B)$ of the \NumMatch problem, we create an instance $\X{J'}=(\Co{A}, \Co{I}, \{\util_{a}\}_{a\in \Co{A}}, \Co{H}, \eta=B)$ of \cffa, where $\Co{I}=X\cup Y\cup Z$ and \Co{H} is a cluster graph on the vertex set \Co{I} with induced cliques on the vertices in the set $X$, $Y$, and  $Z$. We define a set of agents $\Co{A}=\{a_{1}, \ldots, a_{\tilde{m}}\}$ and for each agent $a_{i}\in \Co{A}$, we define the utility function $\util_{a_{i}}(j) = s(j)$ for each \object $j\in \Co{I}$. The proof of correctness of this construction is in the Appendix.


%\todo{construction is almost same as above. So, if we keep the above proof, we need to say this here.}


\begin{dontshow}
\td{Let's move the following claim to Appendix}

\begin{clm}\label{clm:Np-hard-NumMatch}
\X{J} is a \yes-instance of \NumMatch if and only if \X{J'} is a \yes-instance of \cffa

\end{clm}


\begin{proof}Suppose that \X{J} is a \yes-instance of \NumMatch. Then, there is a solution $A_{i}, i\in [\tilde{m}]$, that satisfies the desired properties. It follows then that for the agent $a_{i}\in \Co{A}$, we have the condition that $\sum_{j\in A_{i}}\util_{a_{i}}(j) = \sum_{j\in A_{i}}s(j) =B$. Thus, the assignment function $\phi$, where $\phi(a_i)=A_i$, %$\{A_{i}\mid i\in [m]\}$ 
yields a solution for \X{J'} as well due to the construction of $\Co{H}$. 

Conversely, suppose that we have a solution for \X{J'}, i.e., an assignment function $\phi$ for which $\phi(a_{i}) \cap \phi(a_{j}) = \emptyset$ for every $\{a_{i}, a_{j}\} \sse \Co{A}$, and for every $a_{i}\in \Co{A}$, $\phi(a_i)$ is an independent set and $\sum_{j \in \phi(a_{i})} \util_{a_{i}}(j) \geq B$. %Then, we know that setting $A_{i}=\phi(a_{i})$ will yield the solution if each $\phi(a_{i})$ has size 3. 

%\begin{sloppypar}
Suppose that there exists an agent $a_{i}$ whose bundle $\sum_{j \in \phi(a_{i})} \util_{a_{i}}(j) > B$, then taking all the $\tilde{m}$ bundles together we note that $\sum_{i\in [\tilde{m}]}\sum_{j \in \phi(a_{i})} \util_{a_{i}}(j) > \tilde{m}B$, contradiction to the definition of the problem. Hence, we know that for each agent $a_{i}\in \Co{A}$, $\sum_{j \in \phi(a_{i})} \util_{a_{i}}(j) =B$. Since there are $\tilde{m}$ agents, every \object is assigned to some agent. Furthermore, since $\phi(a_i)$ is an independent set in $\Co{H}$, for each $i\in [\tilde{m}]$, we know that $\phi(a_i)$ contains $3$ elements, one from each clique. Hence, setting $A_{i}= \phi(a_{i})$ gives a solution to \X{J}. 
%\end{sloppypar}
 \end{proof}
\end{dontshow}

This completes the proof. 
\end{proof}
%\end{comment}

%
Next, we show that when the cluster graph has only two cliques and the utility functions are uniform, i.e., for any two agents $a,a'$, $u_a=u_{a'}$, then \cffa can be solved in polynomial time. In particular, we prove \Cref{thm:2cliques}. For arbitrary utility functions, the complexity is open. 
We begin by noting that due to the utility functions being uniform, every bundle is valued equally by every agent. This allows us to look at the problem purely from the perspective of partitioning the \items into $n$ bundles of size at most two.

%\il{*************************Editing here*********************** }

\input{new-file}

\begin{comment}
We define the following polynomial-time solvable problem which  will be used in the proof. 
\defprobgoal{{\sc Matroid Parity}}{a matroid $\Co{M}=(U,\Co{F})$ that is representable over some field $F$, a collection $\Co{P}\subseteq \binom{U}{2}$ of pairs of elements of $U$, and an integer $k$}{find a subset $\Co{S}\subseteq \Co{P}$ of size exactly $k$ such that the set $\cup_{X\in \Co{S}}X$ has size exactly $2k$ and is independent in $\Co{M}$, if it exists, otherwise return ``no''.}

\begin{proposition}[\cite{GabowS86}]\label{prop:MP}
{\sc Matroid Parity} can be solved in polynomial time. 
\end{proposition}
\begin{proof}[Proof of \Cref{thm:2cliques}]
Let $\X{J}=(\A, \I, \{\util_{a}\}_{a\in \A}, \Co{H}, \eta)$  be a given instance of \cffa.
Since the utility functions are uniform, we skip the agent identification from the subscript of utility function, i.e., instead of writing $\util_{a}$ for the utility function of agent $a$, we will only use $\util$. Note that if there exists an item $z$ such that $\util(z) \geq \eta$, then there exists a  solution that assign it to some agent. Since the utility functions are uniform, it can be assigned to any agent. Let $\Co{I}_{\sf HighUtility}\subseteq \Co{I}$ be the set of \items whose utility is at least $\eta$, i.e., $\Co{I}_{\sf HighUtility}=\{z\in \Co{I} \colon \util(z)\geq \eta\}$. Let $\Co{I}_{\sf LowUtility}= \Co{I}\setminus \Co{I}_{\sf HighUtility}$. There are $|\Co{A}|-|\Co{I}_{\sf HighUtility}|$ agents whom we need to assign bundles of size two. Let ${\sf IS}$ be the set of all independent sets of size two in $\Co{H}[\Co{I}_{\sf LowUtility}]$. Since $\Co{H}$ is a cluster graph with 2 cliques, size of ${\sf IS}$ is at most $n^2$. Let $\{x,y\} \in {\sf IS}$. We delete $\{x,y\}$ from ${\sf IS}$ if $\util(x)+\util(y)<\eta$. Now, our goal is to find $|\Co{A}|-|\Co{I}_{\sf HighUtility}|$ disjoint sets from ${\sf IS}$. Towards this, we  reduce to {\sc Matroid Parity} problem. 

\begin{sloppypar}
Formally, the algorithm is as follows: we create $\Co{I}_{\sf HighUtility}$ in polynomial time. Let $\Co{A}' \subseteq \Co{A}$ be a set of size $\min\{|\Co{A}|,|\Co{I}_{\sf HighUtility}|\}$. We assign one item from $\Co{I}_{\sf HighUtility}$ to every agent in $\Co{A}'$. If $\Co{A}' \neq \Co{A}$, then we next create an instance of {\sc Matroid Parity} as follows. 

Let $\Co{M}$ be a uniform matroid with universe $U=\Co{I}_{\sf LowUtility}$, and $\mathcal{F}$ be the subsets of $U$ of size at most $2 (|\Co{A}|-|\Co{I}_{\sf HighUtility}|)$.  It is a representable matroid~\cite{DBLP:journals/tcs/Marx09} of rank at most $2 (|\Co{A}|-|\Co{I}_{\sf HighUtility}|)$. Let $ \Co{P}\subseteq \binom{U}{2} = {\sf IS}$ and $k=|\Co{A}\setminus \Co{A}'|=|\Co{A}|-|\Co{I}_{\sf HighUtility}|$. If $|U|< 2k$, then we return ``no''. 

Otherwise, using \Cref{prop:MP}, we find a subset $\Co{S}\subseteq \Co{P}$ of size $k$, if it exists. If $\Co{S}$ does not exist, then we return ``no''. Otherwise, we assign one set from $\Co{S}$ to every agent in $\Co{A}\setminus \Co{A}'$. Thus, the algorithm runs in polynomial time. 
\end{sloppypar}
%The correctness can be found in supplementary. 
%\begin{comment}
Next, we prove the correctness of the algorithm. If the algorithm returns an assignment of \items to the agents, then clearly, for every agent the utility from the bundle is at least $\eta$. Every bundle is also an independent set in $\Co{H}$ as either we assign bundles of size $1$ or elements of $\Co{S} \subseteq {\sf IS}$. The disjointness is ensured from the fact that $\Co{I}_{\sf HighUtility}\cap \Co{I}_{\sf LowUtility} = \emptyset$, agents in $\Co{A}'$ obtain distinct \items from $\Co{I}_{\sf HighUtility}$, and all the elements of $\Co{S}$ are pairwise disjoint due to the size constraint on $\Co{S}$. In the other direction, suppose that $\phi$ is a solution to $\X{J}$. Let $a$ be an agent whose bundle size is $2$ and $\phi(a)$ contains at least one item from $\Co{I}_{\sf HighUtility}$, say $z$. Update the assignment $\phi$ as follows: $\phi(a)=z$. Note that $\phi$ is still a solution to $\X{J}$.   Let $\Co{A}' \subseteq \Co{A}$ be the set of agents such that for every agent $a\in \Co{A}'$, $|\phi(a)|=1$, i.e., the bundle size assigned to every agent in $\Co{A}'$ is $1$. Clearly, $\phi(\Co{A}')\subseteq \Co{I}_{\sf HighUtility}$. Let ${\sf rem}= \Co{I}_{\sf HighUtility}\setminus \phi(\Co{A}')$. Suppose that ${\sf rem}\neq \emptyset$. Note that \items in ${\sf rem}$ are not assigned to any agent in $\Co{A}$. Let $\Co{A}'' \subseteq \Co{A}\setminus \Co{A}'$ be any set of size $\min\{|\Co{A}\setminus \Co{A}'|,|{\sf rem}|\}$. Let $\Co{A}'' =\{a_1,\ldots,a_\ell\}$ and ${\sf rem}=\{z_1,\ldots,z_q\}$, where $\ell\leq q$. %Clearly, for every $a\in \Co{A}''$, $\phi(a)\subseteq \Co{I}_{\sf LowUtility}$. 
Update the assignment $\phi$ as follows: for every $i\in [\ell]$, $\phi(a_i)=\phi(z_i)$. Clearly, $\phi$ is still a solution of $\X{J}$. If $\Co{A}=\Co{A}'\cup \Co{A}''$, then the algorithm also assigned \items from $\Co{I}_{\sf HighUtility}$ and returned it. Otherwise, let $\Co{\tilde{A}}=\Co{A}\setminus (\Co{A}'\cup \Co{A}'')$. Clearly, every agent in $\Co{\tilde{A}}$ received \items from the set $\Co{I}_{\sf LowUtility}$ and all the \items in $\Co{I}_{\sf HighUtility}$ are assigned to agents in $\Co{A}'\cup \Co{A}''$. Due to our construction of the matroid $\Co{M}$ and $\Co{P}$, all the bundles that are assigned to agents in $\Co{\tilde{A}}$ belong to the set  $\Co{P}$, and $\phi(\Co{{\tilde{A}}})$ is a solution to {\sc Matroid Parity} with $k=|\Co{\tilde{A}}|=|\Co{A}|-|\Co{I}_{\sf HighUtility}|$. Thus, the algorithm in \Cref{prop:MP} return a set $\Co{S}$, and hence our algorithm also returns an assignment. 
\qed \end{proof}
\end{comment}

